A Survey of Challenges for Runtime Verification from Advanced Application Domains (Beyond Software)

Runtime verification is an area of formal methods that studies the dynamic analysis of execution traces against formal specifications. Typically, the two main activities in runtime verification efforts are the process of creating monitors from specifications, and the algorithms for the evaluation of traces against the generated monitors. Other activities involve the instrumentation of the system to generate the trace and the communication between the system under analysis and the monitor. Most of the applications in runtime verification have been focused on the dynamic analysis of software, even though there are many more potential applications to other computational devices and target systems. In this paper we present a collection of challenges for runtime verification extracted from concrete application domains, focusing on the difficulties that must be overcome to tackle these specific challenges. The computational models that characterize these domains require to devise new techniques beyond the current state of the art in runtime verification.

==> 1.distributed/tmp/dist-chara.tex <==
% !TEX root = ../main.tex


\begin{description}
	\item[Heterogeneity and Dynamicity]
	Distributed systems are
notoriously difficult to design, implement and reason about:
%
$(i)$  multiple stakeholders impose their own requirements, which results in disparate specifications expressed in variegated formats and logics that often concern themselves with different layers of abstraction;
%
$(ii)$ implementing them often involves collaboration across multiple development teams and the use of a various technologies;
%
$(iii)$ their sheer size, numerous possible execution interleaving, and unpredictability due to the inherent dynamic nature of the underlying architecture makes distributed systems hard to test and verify using traditional pre-deployment methods.
%
Moreover, distributed computation is often characterised by a high degree of dynamicity where all of the components that comprise the system are not known at deployment (\emph{e.g.,} the dynamic discovery of web-services) --- this dynamicity complicated further system analysis.
  \item[Distributed Clocks and Latency]
  %

  A defining feature of a distributed system is that the execution units making up the underlying structure are often loosely coupled, each having their own computational clock.
  %
  This characteristic is due, in part, to the impracticality of keeping individual clock synchronised with one another: communication latency would drastically slow down computation at the respective locations.
  %
  As a result of this asynchrony, the order of computational events occurring at distinct execution units may not be easy (or even possible) to discern.
  %
  \item[Partial Failure]  A key requirement of any long-running distributed system is that when execution units (occasionally) fail, the overall computation is able to withstand the failure.
  %
  Even in cases where partial failure impacts computation, there is still enough ongoing computation at the residual execution units so as to make it significant and worthwhile \cite{FH08:InfComp}.
  %
  \item[Non-Determinism]
  Fluctuations in latency make is hard to determine unexpected dynamic changes in the underlying architecture  (\emph{e.g.} node failure or message loss).
  %
  In addition, resource availability (\emph{e.g.,} free memory) at individual execution units is hard to anticipate and guarantee.
  %
  This unpredictability, together with computation asynchrony, often induces non-deterministic behaviour in distributed computation.
  %
  \item[Multiple Administrative Domains]
  %
  In a distributed system, computation often crosses administrative boundaries that restrict unfettered computation due to security and trust issues (\emph{e.g.,} untrusted code spawned or downloaded from a different administrative domain may be executed in a sandbox).
  %
  Administrative boundaries also limit the migration and sharing of data across these boundaries for reasons of confidentiality.
  %
  \item[Multiple Accessibility]
  %
  Different components may feature different accessibility when it comes to analysis, maintenance, monitoribility, instrumentation, or enforcement. The connected technologies may range from proprietary to public domain, from available source code to binaries only, from well documented developments to sparsely documented (legacy) systems.
  %
  \item[Multiple Criticality]
  %
  The different components of a distributed system may not be equally critical for the overall mission.  The consequences of malfunctioning of certain components are more severe than than malfunctioning of others. For instance, the failure of one client is potentially less critical than the failure of a server which many clients connect to. Or some components could be critical for preventing data loss, financial loss, or alike, whereas others may `only' affect performance, customer satisfaction, or alike.
  %
  \item[Evolving Requirements]
  %
  The execution of a distributed system is typically characterised by a series of long-running reactive computational entities (\emph{e.g.,} a web server that should ideally never stop handling client requests).
  %
  Such components are often recomposed into different configurations (\emph{e.g.,} service-oriented architectures) where their intended users change.
  %
  In such settings, it is reasonable to expect the correctness specifications and demands to change over the execution of the system, and to be composed of smaller specifications obtained from different users and views.
\end{description}


==> 1.distributed/tmp/dist-existing.tex <==
% !TEX root = ../main.tex


\todo[inline]{Relevant citations are~\cite{sen04efficient,bauer12decentralised,basin13monitoring,basin15failure,cassar16implementing,colombo12polylarva,falcone15runtime,fraigniaud14onthenumber,francalanza13distributed,mostafa15decentralized}.}

\todo[inline]{Basin et al. CAV'17 paper (extension of \cite{basin15failure} to freeze quantifiers)}

\todo[inline]{Check for overlaps with
  Huge data streams (Sect~\ref{sec:huge})}

\todo[inline]{parallelizable algorithms for full LTL~\cite{kuhtz_ltl_2009,kuhtz_efficient_2012} and metric
temporal logic~\cite{bundala_complexity_2014,DBLP:conf/dlt/FengLQ15}}


==> 5.transactions/transactions-old/christianChallenges.tex <==
\subsubsection{Reparation in Transactional Systems}\label{sec:trx:reps}

%
Recovery and reparations in transaction systems  \cite{survey} are multi-layered: If recovering within a transaction action which may still succeed, reparation may be expressed in a \emph{try-catch} fashion. However, if the action is considered to have failed, then any previously completed parts of the transaction would need to be rolled back. This is done to preserve the atomicity of the transaction, i.e., either  entirely succeeds or entirely fails. The problem arises when it is not possible to isolate a transaction with the result that its actions affect other parts of the system before the transaction is committed. This usually happens due to long life of the transaction --- making it infeasible to lock the relevant resources for a long time. 

From a monitoring point of view, this rich availability of reparations brings up interesting challenges and opportunities: 
%
\begin{itemize}
\item 
In non-transactional applications, typically monitors would need to have their own reparation code to be executed in case the monitor flags a problem. In the case of transactional application monitoring, reparations are typically readily available and the monitor would simply need to trigger them.
%
While this is more of an opportunity, the challenge lies in how to improve upon current practises and express the behaviour of reparations formally and succinctly in a
specification language --- similarly to how monitors defined. There have been several works in this regard~\cite{colombo12safer,colombo14comprehensive,colombo13monitor} for example through the use of compensating automata. However, future work can focus on further simplifying the specification language and perhaps providing a library of ready made constructs which developers can use directly.
%
\item
From a more pragmatic point of view, compensations and rollbacks present the challenge of managing historic data values to be used in the reparation code. In this respect runtime monitors can be useful as monitors are typically stateful. Therefore, reparations can be parametrized through the monitors' state, avoiding complex wiring to pass the data around. To the best of our knowledge this approach has not been implemented.
\end{itemize}
 


\subsubsection{Pragmatic Considerations}\label{sec:trx:pragmatic}


Transaction systems typically present a number of challenges through their sheer size, and efficiency concerns. In this section we go through a number of these concerns, highlighting the challenges they present.

\subsubsection{Fast-forwarding through events}: When starting to monitor a transaction
system, one might need to fast-forward through years' worth of past events to quickly start monitoring ``at runtime''. This is also useful
when monitors are significantly changed or crash and need to be
restarted. In general this is not easy to automate as this requires
event abstraction, i.e., some way of processing several events at the
same time~\cite{colombo12fast}.

\subsubsection{Synchronous/asynchronous monitoring:}\todo{JL: online stream processing?!}
%
To avoid affecting the running system, it might be useful to monitor
transactions asynchronously --- allowing the monitor to fall behind
and synchronising only when something suspicious is
detected~\cite{colombo12safer}.
%
Typically transaction systems are decomposable from a verification
point of view since for certain properties verifying different
entities (such as users/credit cards/transactions) can be carried out
independently.
%
This means that while some entities are monitored synchronously,
others might be monitored asynchronously for the same
property. 
%
Similarly, monitoring can be done synchronously/asynchronously for
different properties at the same time. This is discussed further in
the next point.

\subsubsection{Fine-grained overhead control:}
%
One of the main concerns in transaction processing is performance and
introducing monitoring automatically introduces overheads.
%
While this might not be a problem in itself, from experience with
industry, one would typically want to be able to control how much
overheads monitors are allocated.
%
In an ideal world, an administrator should be able to observe how much
overhead each property is generating and be able to turn property
monitoring on and off to manage the overheads.
%
In this context, having the possibility of fast-forwarding monitoring
would enable monitors to be paused and then quickly unpaused (see
earlier point), and having the possibility of switching from synchrony
to asynchrony and back would similarly facilitate such overhead
management.
%
While~\cite{colombo12safer} is a prelude to fine-grained monitor
overhead control, to the best of our knowledge, no work has tried to address this
fully.  
%

\subsubsection{Persistence and resilience of monitors:}
%
As the number and size of monitors grow, the need to persist monitors
also grows such that they do not occupy too much main
memory.
%
Similarly, as the reliance on monitors increases, the wish to have
reliable, fault-tolerant monitors likewise increases.
%
While in the case of simple systems, this might not be hard to
achieve, in real-life industrial systems with high degrees of
concurrency, where monitors share some state amongst each other, the
challenge of persisting monitors and ensuring fault tolerance is much
harder.



==> 5.transactions/transactions-old/concl.tex <==
\subsection{Conclusion}

While transaction systems have been around for decades, they have evolved and --- although modified --- the concept is still used heavily in modern systems. Given the stringent properties such systems are required to fulfil, both in terms of correctness and efficiency, it is unsurprising that a number of challenges present themselves to software runtime verification. 

In this chapter we have reviewed a number of aspects of transactional systems highlighting the open challenges these present. We are confident that given the ever growing importance of such systems, more effort will be directed towards addressing such challenges. 

An interesting development in the near future is expected to be in the area of blockchain technology. It would be interesting to see how this evolution of the transaction concept will create new challenges and opportunities for the runtime verification community. \todo{CC: what do you think of this remark about blockchain? feel free to add/edit}




















==> 5.transactions/transactions-old/intro.tex <==

Computational systems take some data as input, process it, and produce new data as output.
%
Traditionally data was stored locally in a set of disk arrays and would be processed by one or more computing units.  Nowadays, data tends to be offload to geographically distant (and possibly replicated) data centers.
%
No mater if the data is local or remote, its processing certainly have requirements concerning availability and performance.
%
Availability requirements can be addressed by replication and appropriate fault handling.
%
Performance requirements are usually addressed by way of using multiple computing systems processing the data simultaneously, which raises additional requirements on data consistency.
% The data processing phase does certainly have some requirements concerning consistency, availability and performance.
%
The transactional model aims at easing the development of computational systems that preserve data consistency requirements in the presence of concurrent accesses to shared data.

\begin{quote}
  \emph{A business is not in business unless it is successfully processing transactions of some kind.}\quad In Alex Kooijmans et all~\cite{}.
\end{quote}

Computational systems execute programs. A program is a specification of a state machine written in a \emph{programming language}, which describes a behaviour.  If the specification is wrong, or even simply incomplete, the corresponding state machine will describe a behaviour other than the expected.  These deviations between the expected and the observed behaviours are called program errors (or \emph{bugs}).  Program errors may cause faults and failures.

The activity of locating, diagnosing and correcting errors in programs is named \emph{debugging}.

\begin{quote}
  \emph{If debugging is the process of removing bugs, then programming must be the process of putting them in.}\quad Edsger W. Dijkstra.
\end{quote}

Debugging requires a good understanding of both the program's expected behaviour (what it was supposed to do) and the program actual behaviour (what it really does).  Any small increase in the understanding of these factors has strong positive impact in the effectiveness of the (debugging) process.

The understanding of a program's actual behaviour is frequently acquired by observation --- not only of the final results but also intermediate values (the program state) at important key locations.

Sequential programs are easy to observe by probing the program's state.  Probing the program state can be achieved actively by using a state debugger or passively by installing an event monitor that generates a list of relevant events and state values during the program's execution.

Although program probing is an accepted and effective practice for sequential programs, the same is not true for concurrent programs (including both parallel and distributed programs), because concurrent programs are inherently non-deterministic.  And non-deterministic programs suffer from an effect similar to the Heisenberg uncertainty principle\footnote{The Heisenberg uncertainty principle or indeterminacy principle, statement, articulated (1927) by the German physicist Werner Heisenberg, that the position and the velocity of an object cannot both be measured exactly, at the same time, even in theory.} that makes them hard to be observed.  Concurrent programs are frequently sensitive to the scheduling of the concurrent activities, which in turn are influenced even by small timing variations.  Probing a concurrent program to observe its internal state frequently requires additional computation and that will change the timings, and influence the scheduling and the program behaviour.  In summary, the simple act of observing a program may change its scheduling and mask existing errors.

\todo{CC: added the below}
To add to the complexity, transactional systems do not only involve high degrees of concurrency but are also typically characterized by high volumes and strict deadlines to maintain the quality of service to the stakeholders, coupled with stringent correctness requirements. This presents both opportunities for the application of software monitoring as well as challenges. 

In the remainder of this chapter we will discuss the challenges and open issues regarding \emph{monitoring transactional systems} using the following organisation: We first start by looking into the transaction mechanism itself focusing on the numerous forms this may take (Section~\ref{sec:trx:itself}). Next, we turn our focus on the distributed nature of transactional systems as this poses a number of significant challenges to monitoring (Section~\ref{sec:trx:distributed}). 
At this stage, we lower our level of abstraction and focus on monitoring transactional applications, i.e., the applications built on top of the transactional mechanism (Section~\ref{sec:trx:apps}). Finally, the last two subsections (Section~\ref{sec:trx:reps} and ~\ref{sec:trx:pragmatic}) focus on the more pragmatic aspects of transaction monitoring, i.e., on how monitor reparations can be integrated within a transaction system; and how the practical aspects of managing high loads with time constraints challenge the monitoring infrastructure. 


\todo[inline]{JL: Christian, do you think this is enough? Please read and rewrite it at your will, because the text is a still bit crude.}
\todo[inline]{CC: I think this is good but not yet an introduction to (all) the below.. so we have to edit once we get feedback from Cesar}


%
%\subsubsection{Definition}
%
%We consider a monitoring application to fall within this section if there is some
%state which is operated upon through a series of atomic operations. In
%general such systems have the following characteristics:
%
%\paragraph{Isolation:}\todo{JL: Not sure this is the best word!}\todo{how about isolation?}
%%
%Typically transaction systems deal with a number of entities with a
%varying degree of interaction. Example of entities might be account
%holders, banks or payment gateways involved in the transaction, credit
%cards or other payment instruments, etc. This means that as long as
%such entities are independent of each other, their monitoring can
%correspondingly occur independently. This aspect is crucial,
%especially given that monitors introduce overheads and performance is
%typically highly prized in such systems.
%
%\paragraph{Concurrency and Distribution:}
%%
%Given that such systems have some form of shared state and they need
%to support as many operations requests as possible, they typically
%allow concurrency up to some degree---making sure that (whether actual
%or eventual) consistency is maintained. Furthermore, given the size
%such systems may reach, they are frequently distributed across several
%sites to have more resources available.
%
%\paragraph{Performance issues:}
%%
%An aspect which is present in most databases, transaction systems,
%etc, is that of performance. The main concern would be typically that
%of ensuring that the user response time remains adequate in the
%circumstances. Monitors are essentially observers and as such they
%introduce overheads, which, given the typical volume of
%transaction/operations per minute can easily prove to be unacceptable.
%


==> 5.transactions/transactions-old/joaoChallenges.tex <==
\todo{is the following a separate subsection or part of the intro?}

Verification/Monitoring replicated distributed systems using relaxed
consistency models, e.g., eventual consistency, and conflict-free
replicated data
types~\cite{kulahcioglou14towards,meiklejohn14vector,burckhardt14replicated}.
%
Replication is a key-strategy to improve availability and performance
in high contented or geographically distributed systems.
%
Such replicated systems may exhibit strict consistency, where all the
replicas are strictly equivalent and any read always returns the
result of the most recent write, to many forms of weaker consistency
models (where replicas are asymmetric, playing different roles, and
the result of an operation may depend on which replica is used).
%
A currently popular data-centric consistency model is ``Eventual
Consistency'', which assumes a replicated database with many readers
and few updaters, and let replicas diverge for some finite time,
ensuring that they will eventually converge to the same contents
value/contents.
%
Monitoring and healing long-living high-availability applications in
deployment.
%
Long-living applications are not necessarily bug or problem-free.
%
They may have to deal with sporadic although extreme changes in
workload, or with under-tested services/functionalities or code-blocks
that reveal to be still buggy.
%
Monitoring these applications for malfunction is challenging, and
could get inspiration from ``Complex Event Processing'' systems from
Oracle and Microsoft's ``Stream Analytics Query Language''.
%
Use ``AspectJ'' or similar to instrument the application to report its
behavior as a stream of events, that can be processed standard or
custom stream query language.
%
Healing of non-fatal errors could take place by further instrumenting
the application code.
%
Errors related to sequential code can be easily handled by rewriting
the corresponding statement(s)/method(s), while errors related to
concurrency could be handled e.g. by inserting/extending atomic code
blocks.

%all these references are included in the text
%Some references are~\cite{colombo12fast,colombo12safer,colombo14comprehensive,kulahcioglou14towards,meiklejohn14vector,burckhardt14replicated,colombo13monitor}.



% \subsection{Notes from the Meeting in Lisbon}
%
% \begin{tabular}{ll}
% \textbf{Participants} & \textbf{email} \\
% \hline
% João Lourenço & joao.lourenc@fct.unl.pt\\
% Nuno Antunes & nmsa@dei.uc.pt\\
% Boro Jakimovski & boro.jakimovski@finki.ukim.mk\\
% \end{tabular}
%
%
% \todo[inline]{TODO: add references}
%
% We believe this section on Transactions (officially section 5, section 6 in the document)  in its present configuration is more focused on “Monitoring Large and/or Complex Systems” rather than monitoring transactional system.  Consequently, there is a  potential high overlap between this section and section 7 (Huge logs).  Most of the challenges identified in this section are general challenges of ARVI and not specific to transactional systems (i.e., they could be invoked as challenges in other subsections as well).
%
% So we suggest that either the title of the section is changed, or the contents/challenges should be adapted to the Transactional setting.  We are working for the second option. Still… the challenges currently identifies in this section can fit into the last class below (Monitoring Transactional Applications).
%
%
% The transactional system provides an abstraction (and supports its implementation).  One may want to monitor and check/verify that the system has a correct implementation of the abstraction provided (transactions).
 
 
 

%=======================================================
\subsection{Challenge: Monitoring the Transactional System Itself}\label{sec:trx:itself}


Transactional systems use different implementation techniques to enforce exclusive access to the shared data.  Among the most popular we may refer to Locking, Timestamp Ordering, and Optimistic Execution.
 
When using a Locking strategy, every transactions acquires the proper lock on each object before it is allowed to access it (to read or modify it). Any other transaction trying to access that object will have to wait until the first transaction commits and the object in unlocked. Read-intensive workloads may benefit from a two-locking scheme, where transactions acquire a shared or exclusive lock for each object that is respectively read or written. The use of locking may easily lead to deadlocks and the transactional system must prevent or handle them.

Timestamp ordering is popular for multiversioning transactional systems, and the key idea behind the timestamp ordering strategy is to use the transactions' identifiers (T\textsubscript{id}) to precompute their serialization order. Because read operations may read past values (not necessarily the last value of the object), concurrent transactions may read and update the same objects and still succeed as long as they do not violate the pre-defined serialization order based in the T\textsubscript{id}. The correct use of timestamp ordering depends on the correct management of T\textsubscript{id} and in the verification that accesses to objects do not break the serialization order.

Optimistic Execution leverages on the assumption that transactions are unlikely to conflict and transactions do not need to acquire locks on objects that are neither read nor updated. Updates are kept in a private store (\emph{write set}) and, at commit time, the proper locks are acquired and, if the transaction is serializable in the current execution setting, the \emph{write set} is applied to the objects, releasing the locks afterwards. This strategy is also popular in multiversioning transactional systems \todo{CC:seems there is a typo here} reduces the amount of time that a transaction holds locks at the expense of managing read and write sets and a timely validation of the transactions.

The challenges in monitoring the transactional system itself include collecting information to verify that serializable transactions are committed, that non-serializable transactions are aborted, and that no deadlocks occur (when applicable).  Some issues raised by these challenges include:

\begin{itemize}
\item Check/verification of locking policies (which locks are or are not compatible);
\item Identification of violation of data access policies (as imposed by the locking mechanism);
\item Check/verification of compliance to different isolation levels;
\item Identification of deadlock situations;
\item Identification of starvation (one transaction find itself systematically being aborted and restarted due to conflicts with some other transaction);
\item Knowing the transactional scheduler state (which transactions could be running, which ones are actually running, and which ones are currently blocked);
%\item Checking the correct interaction with intermediate layers (such as Hibernate~\cite{hibernate}). % Missing: Hybernate
\end{itemize} 
 \todo{CC: I think it would be ideal to comment here on what has already been done. This also applies to the following}
 
%=======================================================
\subsection{Challenge: Monitoring Distributed Transactional Systems}\label{sec:trx:distributed}

Transactional systems may leverage on distributed systems to distribute the workload and increase the resilience to faults by splitting the data and/or by replicating the data among multiple nodes.

The CAP theorem~\cite{brewer00towards,fox99harvest,gilbert02brewer} states that it is impossible for a distributed data store to simultaneously provide more than two out of the following three guarantees: Consistency, Availability and Partition tolerance.  This has implications on the design and behaviour of the distributed transactional systems.  Even if assuming that the network issues are handled by the communication layer, monitoring such systems raises issues such as:
 
\begin{itemize}
\item Global observations / ordering of events in the distributed system;
\item Validation of the distributed locking process;
\item Observation of distributed commit protocol(s);
\item Monitoring and handling temporary disconnections from one or more nodes of the distributed transactional system.
\end{itemize}
 
 
 
%=======================================================
\subsection{Challenge: Monitoring Transactional Applications}\label{sec:trx:apps}

 
Applications that make use of a centralized or a distributed transactional system, are not free of programming errors themselves.  Example of possible errors include: the scope of a transaction may easily be misdefined and lead do High-Level Data Races~\cite{hldr} or transactions that hardly commit\todo{CC: is it a technical term ``transactions that hardly commit''?}; the transactions enter an infinite loop and never releases the locks held; misidentified dependencies between transactions, which are launched concurrently when they must be executed sequentially.\todo{CC:found it hard to parse the previous sentence}  Monitoring transactional applications raises issues such as:
 
\begin{itemize}
\item Observe dependencies between transactions (separate transactions must be executed in a specific order);
\item Observe misdefined transactions (wrong scope), e.g., the programmer mistakenly split what should have been a single transaction into two (or more) smaller transactions;
\item Observation of long-running transactions (checking if there is progress and no deadlocks);
\item Observation of compensating transactions (a compensation transaction with a set of operations may only occur if it was preceded by a transaction that executed some other specific operations);
\item Observation of data flow/exchange between different transactional systems
\item Application workflow monitoring (to enforce the compliance of the application with a well defined workflow).
\end{itemize}
 
%Seems these references have already been included above~\cite{colombo12fast,colombo12safer,colombo14comprehensive,kulahcioglou14towards,meiklejohn14vector,burckhardt14replicated,colombo13monitor}.

==> 5.transactions/transactions-old/transactions.tex <==
%!TEX root = ../main.tex
%\section{Transactions, Databases, Cloud, Distributed information systems}
\section{Transactional Information Systems}

\input{5.transactions/intro}

\subsection{Challenges}

\input{5.transactions/joaoChallenges}

\input{5.transactions/christianChallenges}



%
\input{5.transactions/concl}


==> 7.huge/huge-cesar.tex <==
% !TEX root = ../main.tex

%\section{Huge data streams and storages, approximate monitoring}
\section{Huge data and approximate monitoring}
\label{sec:huge}

This section describe runtime verification challenges related to the
analysis of very large streams or dumps of data.
%


The general goal when dealing with huge data logs or streams is to
develop algorithms that inhabit the \emph{Pareto-Optimum} of
\emph{scalability}, specification language \emph{expressiveness},
\emph{precision}, and \emph{utility}. 
%
Below we discuss the advances made along each of these dimensions and
outline remaining challenges.

\input{7.huge/scalability}

\subsection{Expressiveness}
\input{7.huge/expressiveness}

\subsection{Precision}
\input{7.huge/precision}


\subsection{Usability}
\DB{the original text by SK says ``Utility'' but the email by DT says ``Usability''}

\input{7.huge/usability}

\todo[inline]{}

\subsection{Challenges}

\begin{challenge}{Expressive Specification Languages}
  \label{ch:expressive}
%
  Richer specification languages allow to capture more sophisticated
  properties.
%
  For example, hyperproperties allow to express relational properties
  (essentially properties that releate different traces). 
%
  These traces can come from a single large dump trace that is
  processed offline.

  For example, a specification can relate two traces, which are
  extracted from the large trace as requests coming from different
  users or different requests performed at different points in time.
%
  These richer language would allow to express properties like
  differential SLA that are beyond the expressivity of the
  specification formalisms currently used.

  Another family of specification languages that allow to express rich
  properties is stream runtime verification languages. 
%
  Currently, these languages only have online and offline evaluation
  algorithms for small traces, in the sense of traces that can be
  stored in a single computer.
\end{challenge}

\begin{challenge}{Richer Verdicts and Concise Model Witnesses}
  \label{ch:verdicts}
%
  Classical specification formalisms from runtime verification
  borrowed from behavioral languages used in static verification
  generate Boolean outcomes from a given trace, which indicate whether
  the trace observed is a model of the specification.
%
  One challenge is to compute richer outcomes of the monitoring
  process.
%
  Examples include computing quantitative verdicts, like for example
  how robustly was the specification satisfied or computing statistics
  from the input trace, like the average number of retransmissions or
  the worst-cae response time.
%
  A related challenge is the computation of witnesses of the
  satisfaction or violaton of the property for offline traces.
%
  The main goal is that the monitoring algorithm computes the verdict
  and as by-product a compressed summary trace, where irrelevant
  information has been omited and consolidated.
%
  Algorithms will have to be created to (1) check that the summary
  trace is indeed a summary of the input trace, and (2) that the
  summary trace has the claimed verdict against the specification.
%
  This process, if successful, will allow to check independently that
  the runtime verification process was correctly performed.
\end{challenge}

%\subsection{(Old) Material by DB}
%\input{7.huge/DB}

% \subsection{Old) Material by ETH}
%\input{7.huge/ETH}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> 7.huge/old-huge/CS.tex <==
\paragraph{Richer Logics}

\todo[inline]{Cite some of the most relevant logics used in monitoring
  large traces offline. Then, justify that richers logics, even logics
  with undecidable decision problems, are always in need, adding
  features like stream runtime verification, parametrization, etc}

%
% Challenges, Sketch (Cesar)
%
Challenges:
\begin{itemize}
\item dealing with large traces
\item checking temporal properties that use large time intervals
\item adapt this the log-splitting framework to the online setting
\item it is an open problem whether there are nontrivial fragments of
  MFOTL that use first-order features and can be monitored in trace
  length independent way
\item logical fragments that can be monitored in event-rate
  independent way.
\item how to handle large traces when monitors face real-time
  constraints that force them to produce timely verdicts
\item generalize the monitoring setting to tune the precision at which
  monitoring is performed and hence provide an explicit tradeoff
  between precision and efficiency
\end{itemize}

%
% Challenges, sketch (Cesar)
%
 Challenges:
\begin{itemize}
\item Richer logics: there is always a need to more and more expressive
  logics. Even though in logics for static verification there is a
  tension between expressivity and tractability/decidability, the
  latter is less important for dynamic analysis. As long as a
  formalism has operational semantics, one can go ahead an create a
  monitor.
\item Find richer "summaries". The outcome of a monitoring activity is
  usually a verdict. Sometimes a model is built (for example for
  FOMTL, quantifiers are instantiated). By summaries we mean small
  evidences of the verdicts. Ideally a summary is much smaller than
  the input trace itself and (a) checking the summary against the
  trace is easy, and (b) checking that the summary is a mode is easy
  as well. Summaries can be seen as concise abstractions (that
  abstract the concrete trace at hand) that provice good explanations
  of why the trace is a model.  
\end{itemize}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> 7.huge/old-huge/DB.tex <==

%
% Background (Domenico)
%


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> 7.huge/old-huge/ETH.tex <==
% !TEX root = ../main.tex
%
% ETH
%



\paragraph{Expressiveness --DT}

There exist trace length independent monitoring algorithms for past
time metric temporal logic~\cite{thati_monitoring_2005} and extensions
of LTL with aggregation
operators~\cite{du_trace-length_2015}. Similarly, efficiently
parallelizable algorithms for full
LTL~\cite{kuhtz_ltl_2009,kuhtz_efficient_2012} and metric temporal
logic~\cite{bundala_complexity_2014,DBLP:conf/dlt/FengLQ15} are known.

\paragraph{Precision --SK}

Soundness

\paragraph{Utility --SK}

Input and Output

Input BDM (distributed)

Output USAF

\todo[inline]{D. Traytel: Text below copied from ``Big Data Monitoring'' proposal: Needs adjustment}
\paragraph{Runtime Verification}

\todo[inline]{Change title of this part to reflect each challenge}

\todo[inline]{Aerial~\cite{aerial_mtl_2017,aerial_mdl_2017}}

\paragraph{Queries on Streams}
\todo[inline]{Change title of this part to reflect each challenge}

\todo[inline]{Criterion: what works with \emph{huge} data?}

Querying high-velocity streams of data is an active research topic
that has yielded numerous data stream management systems
(DSMS)~\cite{abadi_design_2005,abadi_aurora:_2003-1,arasu_stream:_2003,cetintemel_s-store:_2014,chandrasekaran_telegraphcq:_2003,chandrasekaran_telegraphcq:_2003-1,meehan_s-store:_2015}. The
query languages of DSMS are mostly extensions of SQL (e.g., with
window operators~\cite{arasu_cql_2006}), and thus typically much
weaker than logics such as MFOTL due to the absence of proper negation
and more limited capabilities for expressing temporal
relationships. Moreover, DSMS tend to focus on efficient query
execution at the expense of sacrificing a clean semantics of the
property specifications.
The reference model of DSMSs has been defined in the seminal work on
the Continuous Query Language (CQL)~\cite{arasu_cql_2006}. 
In CQL, the processing of streams is split in three steps: first,
stream-to-relation operators -- that is, windows -- select a portion
of each stream thus implicitly creating static database table. 
The actual computation takes place on these tables, using
relation-to-relation (mostly SQL) operators. Finally,
relation-to-stream operators generate new streams from tables, after
data manipulation. Several variants and extensions have been proposed,
but they all rely on the same general processing abstractions defined
above. 

\textit{Complex Event Processing}
(CEP)~\cite{luckham_power_2005,margara_processing_2011} systems are
closely related to DSMS. CEP systems analyze timestamped data streams
by recognizing composite events consisting of multiple atomic events
from the original stream that adhere to certain patterns. The user of
a CEP system controls the analysis by specifying such patterns of
interest. The predominant specification languages for patterns are
descendents of SQL~\cite{gyllstrom_sase:_2006}. An alternative is
given by rule-based languages, such as
Etalis~\cite{anicic_rule-based_2010}, which resemble Prolog. Although
CEP systems improve the ease of specification of temporal
relationships between events over DSMS, they are still significantly
less expressive than MFOTL due to their retricted support for
parametrization of events and lack of quantification over parameters.
Interestingly, some CEP systems use interval
timestamps. In this model, each data element is associated with two
points in time that define the first and the last moment in time in
which it is
valid~\cite{Schultz-Moller:2009:DCE:1619258.1619264,White:2007:NEP:1265530.1265567}.


\textit{Stream reasoning}
is an emerging research area, originating from
the Semantic Web community as a counterpart to DSMS-style stream
querying and processing with a shift of focus towards a clean
semantics~\cite{valle_its_2009}. MFOTL is more expressive than any
query language seriously considered in that area, such as Streaming
SPARQL~\cite{bolles_streaming_2008},
CQELS-QL~\cite{phuoc_native_2011},
C-SPARQL~\cite{barbieri_c-sparql:_2010,barbieri_querying_2010},
SPARQLStream~\cite{calbimonte_enabling_2010},
RSP-QL~\cite{dellaglio_towards_2015}, and
LARS~\cite{beck_lars:_2015}. The achievement of our objectives would
thus be a major advancement in stream reasoning.


\paragraph{Big Data Processing Engines}

This community is responsible for todays revival of stream processing
(the so called second generation stream processing engines)
and many of the above-mentioned communities adapt their approaches to
scale and make use of large heterogeneous computing clusters.
The use of generic frameworks that process massive quantities of data
is likely to be beneficial when monitoring Big Data. Prominent
examples of such frameworks handle Big Data in the online setting by
distributing the computation as in Apache's
S4~\cite{neumeyer_s4:_2010},
Storm~\cite{toshniwal_stormtwitter_2014,noauthor_apache_2016}, Spark
Streaming~\cite{zaharia_spark:_2010,zaharia_discretized_2013} and
Flink (formerly known as
Stratosphere)~\cite{alexandrov_stratosphere_2014}, Google's Cloud
Dataflow~\cite{krishnan_building_2015}, or by cleverly organizing and
reusing the computation of changes as in Differential
Dataflow~\cite{abadi_foundations_2015,mcsherry_differential_2013}. Those
frameworks offer their users a transparent way to parallelize the
computation based on the logical flow of data. Additionally, they
enable rapid deployment of paralallized software on remote distributed
clusters and provide fault tolerance to clusters' node
failures. Different frameworks provide different fault tolerance
guarantees. The weak guarantee ``at most once'' permits the loss of sent
messages. More reliable guarantees are ``at least once'' and ``exactly
once''.

\todo[inline]{Splunk~\cite{Carasso:2012:ES:2424220,Zadrozny:2013:BDA:2517785},
  Flume, MillWheel, Saber, Heron, Kafka Streams, Apache NiFi,
  Apache Samza}

\todo[inline]{Unification
  attempts via reference
  models~\cite{Dindar:2013:MES:2504595.2504726,affetti2017defining,beck_lars:_2015},
Apache Beam (only syntactic)}

\paragraph{Approximate Monitoring}

\todo[inline]{Copied from ``Monitoring at Any Cost'' proposal}

Bartocci at
al.~\cite{DBLP:conf/rv/BartocciGKSSZS12,KalajdzicBSSG13,Stoller2012}
use dynamic knowledge about the event stream to control the amount of
resources that are allocated for monitoring,  which they call overhead
control. They maintain a probabilistic model of the monitored system
and use it to estimate how likely it is for a given temporal property
to be violated in the near future.
The above mentioned approaches all differ in the
probabilistic formalism used to model the monitored
system~\cite{EPTCS124.1}.
The authors, however, focus only on how to obtain a event stream from a
monitored system in a probabilistic way, while the monitoring setting
remains unchanged.

\todo[inline]{More related work on
  adaptive monitoring~\cite{DBLP:conf/wowmom/DenaroMPT05}}
\todo[inline]{More on approx stream
  processing~\cite{Mozafari:2017:AQE:3035918.3056098}}

Over the past two decades, a large number of approximation techniques
have been proposed, that allow for the fast processing of large amounts
of data by trading result accuracy for time and space
complexity. These techniques~\cite{DBLP:conf/propertytesting/2010,DBLP:journals/crossroads/Nelson12}
include sampling, sketches, and on-line aggregation. For example, the
HyperLogLog algorithm~\cite{Flajolet07hyperloglog:the} and probabilistic
databases~\cite{Agarwal.2465355,spoth:2017:cidr:adaptive,mozafarisnappydata}
provide approximate results based on a query's error or response time
constraints.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> 7.huge/out <==
4803b102 (adrianfrancalanza  2017-06-08 14:48:20 +0200  1) % !TEX root = ../main.tex
4803b102 (adrianfrancalanza  2017-06-08 14:48:20 +0200  2) 
4221b49b (Cesar Sanchez      2017-05-18 23:26:48 +0200  3) \section{Huge data streams/storages, approximate monitoring}
37b85f33 (traytel            2017-06-06 14:04:28 +0200  4) \label{sec:huge}
4221b49b (Cesar Sanchez      2017-05-18 23:26:48 +0200  5) 
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100  6) The general goal when dealing with huge data logs or streams is to
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100  7) develop algorithms that inhabit the \emph{Pareto-Optimum} of
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100  8) \emph{scalability}, specification language \emph{expressiveness},
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100  9) \emph{precision}, and \emph{utility}. 
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100 10) %
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100 11) Below we discuss the advances made along each of these dimensions and
00000000 (Not Committed Yet  2018-03-22 15:14:53 +0100 12) outline remaining challenges.
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 13) 
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 14) \input{7.huge/scalability}
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 15) 
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 16) \subsection{Expressiveness}
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 17) 
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 18) \subsection{Precision}
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 19) 
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 20) \subsection{Usability}
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 21) \DB{the original text by SK says ``Utility'' but the email by DT says ``Usability''}
b4ac524f (Domenico Bianculli 2018-03-22 07:30:47 +0100 22) 
803ed314 (Domenico Bianculli 2018-03-22 08:52:51 +0100 23) %\subsection{(Old) Material by DB}
803ed314 (Domenico Bianculli 2018-03-22 08:52:51 +0100 24) %\input{7.huge/DB}
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 25) 
803ed314 (Domenico Bianculli 2018-03-22 08:52:51 +0100 26) \subsection{(Old) Material by CS}
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 27) 
fd5a9a41 (Cesar Sanchez      2017-12-22 16:15:12 +0100 28) \input{7.huge/CS}
37b85f33 (traytel            2017-06-06 14:04:28 +0200 29) 
803ed314 (Domenico Bianculli 2018-03-22 08:52:51 +0100 30) \subsection{Old) Material by ETH}
f2753b3b (Domenico Bianculli 2018-03-09 07:04:30 +0100 31) 
fd5a9a41 (Cesar Sanchez      2017-12-22 16:15:12 +0100 32) \input{7.huge/ETH}
9cb07200 (Srdjan Krstic      2017-06-07 10:53:31 +0200 33) 
9cb07200 (Srdjan Krstic      2017-06-07 10:53:31 +0200 34) %%% Local Variables:
9cb07200 (Srdjan Krstic      2017-06-07 10:53:31 +0200 35) %%% mode: latex
9cb07200 (Srdjan Krstic      2017-06-07 10:53:31 +0200 36) %%% TeX-master: "../main"
9cb07200 (Srdjan Krstic      2017-06-07 10:53:31 +0200 37) %%% End:


==> acm-stuff.tex <==
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}

% Metadata Information
\acmJournal{POMACS}
\acmVolume{9}
\acmNumber{4}
\acmArticle{39}
\acmYear{2010}
\acmMonth{3}
\acmArticleSeq{11}

% Copyright
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}

% DOI
\acmDOI{0000001.0000001}

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>  
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

%
% End generated code
%

